Factorization and pseudofactorization of weighted graphs

For unweighted graphs, finding isometric embeddings is closely related to decompositions of $G$ into Cartesian products of smaller graphs. When $G$ is isomorphic to a Cartesian graph product, we call the factors of this product a factorization of $G$. When $G$ is isomorphic to an isometric subgraph of a Cartesian graph product, we call those factors a pseudofactorization of $G$. Prior work has shown that an unweighted graph's pseudofactorization can be used to generate a canonical isometric embedding into a product of the smallest possible pseudofactors. However, for arbitrary weighted graphs, which represent a richer variety of metric spaces, methods for finding isometric embeddings or determining their existence remain elusive, and indeed pseudofactorization and factorization have not previously been extended to this context. In this work, we address the problem of finding the factorization and pseudofactorization of a weighted graph $G$, where $G$ satisfies the property that every edge constitutes a shortest path between its endpoints. We term such graphs minimal graphs, noting that every graph can be made minimal by removing edges not affecting its path metric. We generalize pseudofactorization and factorization to minimal graphs and develop new proof techniques that extend the previously proposed algorithms due to Graham and Winkler [Graham and Winkler, '85] and Feder [Feder, '92] for pseudofactorization and factorization of unweighted graphs. We show that any $m$-edge, $n$-vertex graph with positive integer edge weights can be factored in $O(m^2)$ time, plus the time to find all pairs shortest paths (APSP) distances in a weighted graph, resulting in an overall running time of $O(m^2+n^2\log\log n)$ time. We also show that a pseudofactorization for such a graph can be computed in $O(mn)$ time, plus the time to solve APSP, resulting in an $O(mn+n^2\log\log n)$ running time.

==> factor-background.tex <==
% A graph $G=(V,E,w_G)$ consists of a set of nodes, denoted $V$ or $V(G)$, connected by a set of edges, denoted $E$ or $E(G)$, with a weight function $w_G:E\rightarrow \mathbb{R}$. For the purpose of this proposal, all graphs are undirected, and I will denote edges as $e=\{u,v\}=uv$ where $u$ and $v$ are the endpoints of edge $e$. The function $d_G$ denotes graph distance such that $d_G(u,v)=\min_P\{\sum_{e\in P}w_G(e)\}$  where $P$ is any set of edges forming a path from $u$ to $v$. Unless otherwise noted, we take $G$ to be an unweighted graph, meaning $w_G(e)=1$ for all $e\in E(G)$ and we take $kG$ to be a uniformly weighted graph with weight $k$, meaning $w_{kG}(e)=k$ for all $e\in E(kG)$. This means $d_{kG}=kd_G$. In either of these cases, we may omit the weight function and write $G=(V,E)$ when describing the graph.  

% An \textit{isometric embedding} from $G_1$ to $G_2$ is a mapping $\alpha:V(G_1)\rightarrow V(G_2)$ such that $d_{G_1}(u,v)=d_{G_2}(\alpha(u),\alpha(v))$ for all $u,v\in V(G_1)$. We define an \textit{isomorphism} between $G_1$ and $G_2$ as a bijection $\alpha:V(G_1)\rightarrow V(G_2)$ such that $\alpha(u)\alpha(v)\in E(G_2)$ if and only if $uv\in E(G_1)$ and $w_{G_2}(\alpha(u)\alpha(v))=w_{G_1}(uv)$ for all $uv\in E(G_1)$. We call two graphs \textit{isomorphic} if there exists an isomorphism between them. We also note that if two graphs are unweighted, they are isomorphic if and only if there exists a bijective isometric embedding between them. 
% In this section, 
% % Using these definitions, 
% we discuss several characteristics of isometric graph embeddings.

% Because certain concepts are essential to this section, we reiterate some of the definitions given in Chapter 1. In particular, the Cartesian product of two graphs, $G_1,G_2$, is the graph $G=G_1 \times G_2$ where:
% $$
% V(G) = \{(u_1,u_2)\ | \ u_1\in V(G_1),u_2\in V(G_2)\}
% $$
% % $$
% V(G) = V(G_1)\cartprod V(G_2)
% $$
% $$
% E(G) = \{(u_1,u_2)(v_1,v_2) \suchthat (u_1=v_1 \text{ and } u_2v_2\in E(G_2))\text{ or }(u_2=v_2\text{ and }u_1v_1\in E(G_1))\}
% $$
% For a product of $m$ graphs $G=G_1\cartprod G_2\cartprod ...\cartprod G_m=\Pi_{i=1}^mG_i$, we have:
% $$
% V(G) = \{(u_1,u_2,...,u_m) \suchthat \forall i,u_i\in V(G_i)\}
% $$
% $$
% V(G) = V(G_1)\cartprod V(G_2)\cartprod...\cartprod V(G_t)
% $$
% $$
% E(G) = \{(u_1,u_2,...,u_m)(v_1,v_2,...,v_m) \suchthat \exists i \text{ such that } u_iv_i\in E(G_i) \text{ and } \forall j\neq i, u_j=v_j  \}
% $$

In Figure \ref{fig:factor}, we have that subfigure (a) is the Cartesian product of the graphs in subfigure (b). The Cartesian product of $m$ graphs can be found in polynomial time in the size of the product graph (although the size of the product graph may be exponential in the size of the factor graphs). 
% A \textit{factorization} of a graph $G$ is a set of factor graphs $G_i$ such that $\Pi_iG_i$ is isomorphic to $G$. $G$ is \textit{prime} if its only factorizations consist of $G$ itself and $K_1$. A \textit{prime factorization} is a factorization of $G$ such that all of the factors are prime. 
We will assume that a factorization never includes $K_1$ unless the graph being factored is $K_1$ (so a factorization of a prime graph would only include itself). 
% When the graph is connected, this process turns out to take linear time in the size of the input. 
Imrich and Klav\v{z}ar \cite{ImrichHammingRecognize} showed that deciding if a graph's prime factorization consists entirely of complete graphs can be done in as little as $O(|E|)$ time. More recently, Imrich and Peterin \cite{imrichLinearFactoring} showed that finding the prime factorization of an arbitrary unweighted, connected graphs can also be done in as little as $O(|E|)$ time. However, if the input graph is not connected, this problem is at least as hard as graph isomorphism, which is not known to be in P. We can see this by considering two connected graphs $G,H$, and noting that $G\cup H$ has the graph of two unconnected nodes as a factor if and only if $G$ and $H$ are isomorphic \cite{DezaLaurentText3}.

% as the graph of two unconnected nodes is a factor of the union of two connected graphs if and only if the two graphs are isomorphic.
The concept of graph factorization can be extended by considering isometric embeddings of graphs into the Cartesian products of other graphs, forming a concept we call \textit{pseudofactorizations}. \input{pseudofactorization-background}

% (This discussion largely follows the concepts discussed by Graham and Winkler in \cite{graham1985isometric} but I have opted for a slight change in terminology in order to avoid confusion with the concept of factorization as introduced above.)
% % is what Graham and Winkler refer to in their discussion on a \textit{canonical embedding} and \textit{canonical factor graphs} \cite{graham1985isometric}. However, to avoid confusion with factorization, as defined above, I will opt for a slight change in notation and refer to the concept of pseudofactorization.
% Given a graph $G$ that is isometrically embeddable in the Cartesian product of graphs $G_i$, we write that $G\hookrightarrow \Pi_{i=1}^tG_i$ where $\hookrightarrow$ denotes ``can be isometrically embedded into." 
% % and we call the $G_i$ \textit{pseudofactors} of $G$ if for each $u_i\in G_i$, the . 
% We will call $\{G_1,G_2,...,G_t\}$ a pseudofactorization of $G$ if and only if
% there exists an isometric embedding $\alpha:V(G)\rightarrow V(\Pi_{i=1}^tG_i)$ with $\alpha(u)=(\alpha^1(u),\alpha^2(u),...,\alpha^t(u))$ meeting the following criteria:

% \begin{enumerate}[(i)]
%     \item $G_i\neq K_1$ for all $G_i$ (unless $G=K_1$)
%     \item $\forall u_i\in V(G_i),\exists u\in V(G)$ such that $\alpha^i(u)=u_i$
% \end{enumerate}
% $\exists u\in V(G)$ with $\alpha^i(u)=u_i$, we will call the set of $G_i$ a \textit{pseudofactorization} of $G$. 
% As noted by Winkler, an alternative way of stating (ii) is  that
% % , if the set of $G_i$ is a pseudofactorization of $G$, then 
% each node in each graph must appear at least once as a coordinate in the image of an isometric embedding of $G$ into the Cartesian product of the $G_i$ \cite{winkler1987metric}. This ensures that the $G_i$ are never larger than $G$ itself. 

% $G_i$ \textit{pseudofactors} of $G$. In other words, $G_i$ is a pseudofactor of $G$ if there exists an isometric embedding, $\alpha$, of $G$ into a Cartesian product including $G_i$ such that $G_i$ appears at least once as a coordinate in the image of $\alpha$.
% If $G\hookrightarrow \Pi_{i=1}^t G_i$ and all the $G_i$ are pseudofactors of $G$, then the set of $G_i$ is a pseudofactorization of $G$. 
% We can note that, unlike factors of $G$, pseudofactors can actually be larger graphs than $G$ itself. 


% For ease of notation, if $\alpha: G \rightarrow \Pi_{i=1}^tG_i$ is an isometric embedding, we will let $\alpha(u)=(\alpha_1(u),\alpha_2(u),...,\alpha_t(u))$.  
% We consider the set of 
% % the canonical embedding of a graph, $G\neq K_1$ into its set of
% \textit{canonical pseudofactor graphs} 
% We will call a graph $G$ an \textit{irreducible graph} if all pseudofactorizations of $G$ consist of only $G$ itself. We additionally call a pseudofactorization $\{G_1,G_2,...,G_t\}$ of a graph $G$ an \textit{irreducible pseudofactorization} if each $G_i$ is irreducible. Being irreducible in the context of pseudofactorization is analogous to being prime in the context of factorization.
% there there exists the isometric embedding $\alpha: V(G) \rightarrow V(\Pi_{i=1}^tG_i)$  
% meeting these three criteria 
% \begin{center}
%     \begin{enumerate}[i]
%     \item $G_i\neq K_1$ for all $i$ 
%     \item $\forall u_i\in V(G_i),\exists u\in V(G)$ such that $\alpha^i(u)=u_i$ (The $G_i$ form a pseudofactorization.)
%     \item Each $G_i$ is \textit{irreducible}
% \end{enumerate}
% \end{center}
% If an embedding meets criteria (i) and (ii), it is \textit{irredundant}. A graph, $G$, is \textit{irreducible} if all irredundant isometric embeddings of $G$ into the Cartesian product of graphs are automorphisms. (We also take $K_1$ to be an irreducible graph.) 


Two interesting problems emerge related to the concept of graph pseudofactorization: that of determining if a given graph $G$ is irreducible and that of finding the canonical pseudofactorization of $G$. It turns out that in the case of connected unweighted graphs both of these questions can be answered in as little as $O(|V||E|)$ time \cite{feder} but that finding an irreducible pseudofactorization for an unconnected graph is likely hard for the same reasons that factorization is. Figure \ref{fig:factor}(c) shows the canonical pseudofactorization of Figure \ref{fig:factor}(a).

\begin{figure}

\centering
\includegraphics[width=.4\linewidth]{figures/factor2.png}

\caption[An example of factorization and pseudofactorization]{ Subfigure (a) shows a non-prime, non-irreducible graph. Subfigure (b) shows the prime factorization of the graph in (a). Subfigure (c) shows the canonical pseudofactorization of the graph in (a).}
\label{fig:factor}
\end{figure}

==> factorization-background.tex <==
% \subsection{Cartesian products and factorization}



In order to discuss graph embeddings, we will first discuss Cartesian products of graphs, which we define formally with Definitions \ref{def:cart-prod-unw} and \ref{def:cart-prod-weighted}. 

\begin{definition}\label{def:cart-prod-unw}
For two \textbf{unweighted} graphs $G_1=(V_1,E_1)$ and $G_2=(V_2,E_2)$, the \textbf{Cartesian product} of the graphs, $G_1\times G_2$ is a graph $G=(V,E)$ with vertex and edge sets defined as:
\begin{align*}
    V &= \{(u_1,u_2) \ | \ u_1\in V_1, u_2\in V_2\} \\
    E &= \{(u_1,u_2)(v_1,v_2) \ | \ \text{either } u_1=v_1 \text{ and } u_2v_2\in E_2 \text{ or } u_2=v_2 \text{ and } u_1v_1\in E_1\}.
\end{align*}
\end{definition}

We will denote the Cartesian product of $m$ graphs as $G_1\times G_2\times \ldots \times G_m$ or $\Pi_{i=1}^mG_i$. Using Definition \ref{def:cart-prod-unw}, we can see that for a graph $G=(V,E)=\Pi_{i=1}^mG_i$, the vertex and edge sets are defined as:
\begin{align}
    V &= \{(u_1,u_2,...,u_m)\ | \ u_1\in V_1, u_2 \in V_2, \ldots , u_k \in V_m\} \\
    &= V_1\times V_2 \times \ldots \times V_m \\
    E &= \{ (u_1,u_2,...,u_m)(v_1,v_2,...,v_m)\ | \ \exists \text{ exactly one } \ell \text{ such that } u_\ell v_\ell \in E_\ell \text{ and for all } i\neq \ell, u_i=v_i\}. \label{eqn:edges-cart-prod}
\end{align}

Figure \ref{fig:basic-cart-prod} shows an example of a Cartesian product of two graphs. We call $G_1,G_2,\ldots,G_m$  \textit{factors} of $G$ because for each $G_i$ there exists a graph such that the Cartesian product of that graph with $G_i$ produces a graph isomorphic to $G$. If a graph $G$ is such that its only factors are itself and $K_1$, we call that graph \textit{prime}. A set of prime graphs $\{G_1,G_2,...,G_m\}$ such that $\Pi_{i=1}^mG_i$ is isomorphic to $G$ is a \textit{prime factorization} of $G$.
% , which was shown by [to do] to be unique for every unweighted $G$.

\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{figures/basic-cart-prod.png}
    \caption[An example of a Cartesian product]{The graph on the right is the Cartesian product of the graphs on the left. The parent edge of a given edge in the product graph is the edge in a factor that has the same color as it. For example, edges $(a,x)(a,y)$, $(b,x)(b,y)$, and $(c,x)(c,y)$ in the product graph all have edge $xy$ in the second factor as their parent edge.}
    \label{fig:basic-cart-prod}
\end{figure}

Looking at equation (\ref{eqn:edges-cart-prod}), we see that every edge in a product graph ``corresponds'' to an edge in exactly one factor graph. We formalize this intuition in Definition \ref{def:parent-edge}.

\begin{definition}\label{def:parent-edge}
Consider a graph $G=(V,E)$ with a factorization $\{G_1,G_2,...,G_m\}$ and an edge $uv\in E$. We will take $u=(u_1,u_2,\ldots ,u_m)$ and $v=(v_1,v_2,\ldots, v_m)$ where $u_i,v_i\in V_i$. By the definition of the edge set of a Cartesian product, there exists exactly one $\ell$ such that $u_\ell\neq v_\ell$, and we must have $u_\ell v_\ell \in E_\ell$. We consider $u_\ell v_\ell$ (an edge in $G_\ell$) to be the \textbf{parent edge} of edge $uv$ in $G$ for the given factorization.
\end{definition}

Using the notion of a parent edge, we will extend our definition in \ref{def:cart-prod-unw} to apply to weighted graphs as well.

\begin{definition}\label{def:cart-prod-weighted}
For two graphs $G_1=(V_1,E_1,w_1)$ and $G_2=(V_2,E_2,w_2)$, we take the \textbf{Cartesian product} $G_1\times G_2$ to be $G=(V,E,w)$ where $V$ and $E$ are exactly as defined in Definition \ref{def:cart-prod-unw}. Additionally, for $(u_1,u_2)(v_1,v_2)=uv\in E$, $w(uv)$ equals $w_i(u_iv_i)$ where $u_iv_i$ is the parent edge of $uv$ in the given factorization of $G$.
\end{definition}

The Cartesian product of graphs has an important property about its distance metric. For two nodes $(u_1,u_2),(v_1,v_2)$ in a Cartesian product $G_1\times G_2$, we can write $d_{G_1\times G_2}((u_1,u_2),(v_1,v_2))=\sum_{i=1}^2d_{G_i}(u_i,v_i)$. To see that $d_{G_1\times G_2}((u_1,u_2),(v_1,v_2))\leq\sum_{i=1}^2d_{G_i}(u_i,v_i)$, we can consider a path composed of a shortest path from $(u_1,u_2)$ to $(v_1,u_2)\in V(G_1\times G_2)$ and a shortest path from $(v_1,u_2)$ to $(v_1,v_2)$. We see that to get this path we can follow a path of edges whose parents form a shortest path from $u_1$ to $v_1$ in $G_1$ and then a path of edges whose parents form a shortest path from $u_2$ to $v_2$ in $G_2$. To see $d_{G_1\times G_2}((u_1,u_2),(v_1,v_2))\geq\sum_{i=1}^2d_{G_i}(u_i,v_i)$, we take a path from $(u_1,u_2)$ to $(v_1,v_2)$ in $G_1\times G_2$ and we see that the path formed in $G_1$ (respectively $G_2$) by the edge parents in $G_1$ (respectively $G_2$) is a path from $u_1$ to $v_1$ in $G_1$ (respectively $u_2$ to $v_2$ in $G_2$). This relationship between the distance metric of a Cartesian product and its factors extends to larger products, so that we have:
\begin{align*}
    d_{\Pi_{i=1}^mG_i}((u_1,\ldots,u_m)(v_1,\ldots,v_m))=\sum_{i=1}^md_{G_i}(u_i,v_i).
\end{align*}
These definitions will help us in defining factorization and pseudofactorization in Sections 3 and 5 and in gaining a more complete understanding of hypercube embeddings in Section 4.


==> graph-definitions.tex <==
Throughout this paper, we will consider unweighted and weighted graphs. An unweighted graph $G=(V,E)$ consists of a set of vertices $V$ and a set of edges $E$. We will also use $V(G)$ and $E(G)$ to denote the vertices and edges of a graph $G$, respectively. We will generally denote vertices using a letter or a tuple. For the purposes of this paper, all graphs will be assumed to be undirected, meaning that the edges in the graph have no direction and the distance between any pair of nodes is the same in either direction. We will denote an edge between two vertices $u$ and $v$ as $\{u,v\}$, $uv$, or $vu$. In the case of weighted graphs, we also have a \textit{weight function} on the edges which assigns a positive number to each edge in the graph. For these graphs, we will generally write $G=(V,E,w)$ where $w$ is the weight function in question. For a general weighted graph $G$, we may also write $w_{G}$ to denote the weight function of $G$.  

We will denote the shortest path distance function associated with a graph as $d_G(\cdot,\cdot)$ (or just $d(\cdot,\cdot)$ if the graph in question is implicit). We will also work with graph embeddings, namely \textit{isometric graph embeddings}. Informally, an isometric embedding from one graph into another is a map from the vertices of the first graph to the second such that the distance between vertices in the first graph is preserved under the mapping to the second graph. Formally, an isometric embedding of a graph $G$ into a graph $G'$ is a mapping $\pi: V(G)\rightarrow V(G')$ such that for each $u,v\in V(G)$, $d_G(u,v)=d_{G'}(\pi(u),\pi(v))$. 


==> hamming-embeddings-structure.tex <==

For unweighted graphs, previous work by Graham and Winkler \cite{graham1985isometric} showed a surprising result: Any unweighted graph $G$ has a unique set of irreducible pseudofactor graphs $\{G_1, \dots, G_{n}\}$ for which $G$ is isometrically embeddable into $\prod_{i=1}^{n} G_i$ and with the property that, for any other isometric embedding into $\prod_{j=1}^{m} H_j$, each $H_j$ is isometrically embeddable into a product of one or more $G_i$. Because the irreducible pseudofactorization of $G$ is unique, we call this set the \emph{canonical pseudofactors}. In fact, for unweighted graphs, the corresponding isometric embedding of $G$ into the product of its canonical pseudofactors is also unique up to symmetries of the pseudofactor graphs, and Graham and Winkler refer to this embedding as the \emph{canonical embedding} $\pi$ of $G$, $\pi : V(G) \to V(\prod_{i=1}^{n} G_i)$.

With weighted graphs, although irreducible pseudofactorization is still unique, the uniqueness of isometric embedding no longer holds (for example, see Figure \ref{fig:weighted-graphs}c). In this section, we show that the pseudofactorization of weighted graphs has implications for the structure of its isometric embeddings into Hamming graphs. This partially extends Graham and Winkler's results on unweighted graphs to Hamming embeddings of weighted graphs. Specifically, we show that any weighted graph $G$ permits a Hamming embedding if and only if each of its pseudofactors permits a Hamming embedding.

We introduce the following notation for this section. For embedding $\eta : V(G) \to V(H)$, if $H$ is a Hamming graph then $V(H) = \Sigma^m$, where $\Sigma$ is the alphabet and $m$ the dimension of $\eta$, and distance in $H$ is given by the Hamming distance between pairs of vertices. When $\eta$ is isometric and $H$ is a Hamming graph or hypercube (i.e. $|\Sigma|$ = 2), we say $\eta$ is a Hamming embedding or hypercube embedding, respectively. We use subscripts to refer to individual letters in the image of $\eta = (\eta_1, \dots, \eta_m)$ or, equivalently, $\eta = \eta_1\cdots\eta_m$. The indices $[m]$ of $\eta$ are its \emph{coordinates}, where $[m]$ is the first $m$ positive integers, and each letter $\eta_i$, $1\le i \le m$, is a \emph{digit}. Two Hamming embeddings $\eta$, $\eta'$ are equivalent if there exists a permutation $\sigma$ of the $m$ coordinates and $m$ functions $\beta_i$, $1\le i\le m$, such that $\eta'(u) = \beta_1(\eta_{\sigma(1)}(u))\cdots \beta_m(\eta_{\sigma(m)}(u))$ for all $u \in V(G)$. A Hamming embedding of $G$ is unique if it is equivalent to all other Hamming embeddings of $G$. We assume there are no unnecessary digits in $\eta$ (i.e. every digit changes across some edge), which is analogous to our assumption in earlier sections that $K_1$ is not used in any factorization or pseudofactorization.

For any two vertices $u,v \in V(G)$, we define the function $D_\eta$ as follows:
\begin{equation}\label{eqn:coorddiff}
\coorddiff{\eta}{u}{v} = \{ j \in [m] : \eta_j(u) \ne \eta_j(v) \},
\end{equation}
noting that distance in a graph $G$ with Hamming embedding $\eta : V(G) \to V(H)$ implies that $d_G(u,v) = d_\eta(u,v) = |D_\eta(u,v)|$, where $d_\eta(u,v):=d_H(\eta(u),\eta(v))$. When $uv$ is an edge, we say that the digits corresponding to the elements of $D_\eta(u,v)$ change across $uv$. We also introduce a relation $\gamma$, which relates two coordinates of an embedding if there is some edge across which both corresponding digits change value:
\begin{equation}\label{eqn:gamma}
j \gammarel j' \iff \exists uv \in E(G), \{j,j'\} \subseteq \coorddiff{\eta}{u}{v}.
\end{equation}
Let $\gammahrel$ be the transitive closure of $\gamma$. We know that $\gamma$ is symmetric and reflexive, so $\gammahrel$ is an equivalence relation. 

A \emph{partition} $\{\eta^1, \dots, \eta^{n}\}$ of an $m$-dimensional Hamming embedding $\eta$ is defined by a partition of its coordinates $[m]$, $\{J_1, \dots, J_{n}\}$, with each $\eta^i$ equal to the projection of $\eta$ onto the coordinates in $J_i$.  Let $[m]/\hat\gamma$ be the equivalence classes of $[m]$ under $\hat\gamma$. Then $[m]/\hat\gamma$ defines a partition of $\eta$, which we call its \emph{canonical partition}. This terminology is motivated by Theorem \ref{thm:bijection}, which guarantees a bijection between the canonical partition of $\eta$ and the set of canonical pseudofactors of $G$.

In this section, we begin by constructing a bijection between the canonical partition of any Hamming embedding of $G$ and its set of canonical pseudofactors. Then Theorem \ref{thm:structure} uses this result to prove that $G$ permits a Hamming embedding if and only if each of its pseudofactors also permits a Hamming embedding, which is the main result of this section.


\begin{lem}\label{lem:structure:1}
Let $G$ be a weighted graph and $\eta$ a Hamming embedding of $G$. Let $uv, u'v' \in E(G)$, $j \in \coorddiff{\eta}{u}{v}$, and $j' \in \coorddiff{\eta}{u'}{v'}$. Then we have
\[ uv \thetahrel u'v' \iff j \gammahrel j'. \] 
\end{lem}

\begin{proof}
To see that $uv \thetahrel u'v' \Rightarrow j \gammahrel j'$, observe that $j \notgammahrel j'$ implies that $\coorddiff{\eta}{u}{v}$ and $\coorddiff{\eta}{u'}{v'}$ are disjoint. Thus,
\begin{multline*}
\edgediff{G}{u}{v}{u'}{v'} \\
= \sum_{s \in [m]} \edgediff{\eta_s}{u}{v}{u'}{v'} = 0
\end{multline*}
because each summand is nonzero only if both $\eta_s(u) \ne \eta_s(v)$ and $\eta_s(u') \ne \eta_s(v')$. So $j \notgammahrel j' \Rightarrow uv \notthetarel u'v'$, and $uv \thetarel u'v' \Rightarrow j \gammahrel j'$. If instead $uv \thetahrel u'v'$ then some sequence of edges $(e_i)_{i = 1}^l$ satisifes $uv \thetarel e_1 \thetarel \cdots \thetarel e_{l} \thetarel u'v'$, and the transitivity of $\gammahrel$ implies $j \gammahrel j'$.

To prove $j \gammahrel j' \Rightarrow uv \thetahrel u'v'$, let $S = \coorddiff{\eta}{u}{v} \cap \coorddiff{\eta}{u'}{v'}$, the set of all coordinates that change across both $uv$ and $u'v'$. We prove the statement in two cases:

\begin{description}
\item[Case 1 ($|S| > 0$):] Consider any path $P$ with $l$ edges, beginning with $uv$ and ending with $u'v'$, $l \ge 2$. We show by induction on $l$ that $|S| > 0 \Rightarrow uv \thetahrel u'v'$. As a base case, consider $l=2$ and without loss of generality let $P = (u, v=u', v')$. As above, we consider
\begin{multline*}
\edgediff{\eta}{u}{v}{u'}{v'} \\= \sum_{s \in S} \edgediff{\eta_s}{u}{v}{u'}{v'}
\end{multline*}
with the sum restricted to coordinates $s \in S$ for which the summand is nonzero. Because $v=u'$, $\eta_s(v) = \eta_s(u')$, so $d_{\eta_s}(v,u') = 0$ and $d_{\eta_s}(u,u') = d_{\eta_s}(v,v') = 1$. Thus, each summand is at least +1 and the summation is at least $+|S|$ and $|S| > 0 \Rightarrow uv \thetarel u'v'$. Now, consider the case $l > 2$ and $P = (u_0 = u, u_1 = v, \dots, u_{l-1}=u', u_{l}=v')$. If every edge $u_{i-1}u_i$, $1 < i < l$, has $S$ and $ \coorddiff{\eta}{u_{i-1}}{u_i}$ disjoint, then $\eta_s(v) = \eta_s(u')$ for all $s\in S$ and as in the base case we have $|S| > 0 \Rightarrow uv \thetarel u'v'$. If some edge $u_{i-1}u_i$ has $S$ and $\coorddiff{\eta}{u_{i-1}}{u_i}$ not disjoint, then consider the subpaths $P_1 = (u_0, u_1, \dots, u_{i})$ and $P_2 = (u_{i-1}, u_i, \dots, u_l)$, with $l_1$ and $l_2$ edges, respectively. Clearly $2 \le l_1, l_2 < l$, so by induction we conclude that $uv \thetahrel u_{i-1}u_i \thetahrel u'v'$.
\item[Case 2 ($|S| = 0$):] We are given $j \gammahrel j'$, so construct a sequence of coordinates $j_0 = j, \dots, j_l = j'$ such that $j_{i-1} \gammarel j_i$ for all $1 \le i \le l$. For each pair of coordinates $j_{i-1}$, $j_i$ there is some edge $e_i$ across which both $\eta_{j_{i-1}}$ and $\eta_{j_i}$ change. By Case 1, we have $uv \thetahrel e_1$, $e_l \thetahrel u'v'$, and $e_{i-1} \thetahrel e_i$ for $1 < i \le l$. Thus, $uv \thetahrel u'v'$ as desired. 
% \qedhere
\end{description}
\end{proof}


\begin{thm}
\label{thm:bijection}
Let $G$ be a weighted graph and $\eta$ an $m$-dimensional Hamming embedding of $G$. Then there is a bijection between $E(G) / \hat\theta$ and $[m] / \hat\gamma$. It follows that there is a natural bijection from the set of canonical pseudofactors of $G$ to the canonical partition of $\eta$.
\end{thm}

\begin{proof}
We first construct a bijection from $E(G)/\hat\theta$ to $[m]/\hat\gamma$. Let $[uv]_{\hat\theta} \in E(G)/\hat\theta$ contain $uv \in E(G)$ and $[j]_{\hat\gamma} \in [m]/\hat\gamma$ contain $j \in [m]$. Then we consider the mapping $f_2 : [uv]_{\hat\theta} \mapsto [j]_{\hat\theta}$ where $j \in \coorddiff{\eta}{u}{v}$. By Lemma \ref{lem:structure:1}, $f_2$ is injective because for  $j \in \coorddiff{\eta}{u}{v}$ and $j' \in \coorddiff{\eta}{u'}{v'}$, $f_2([uv]_{\hat\theta}) = f_2([u'v']_{\hat\theta})$ implies $[j]_{\hat\gamma} = [j']_{\hat\gamma}$, so $j \gammahrel j'$ and thus $uv \thetahrel u'v'$. $f_2$ is surjective because each digit of $\eta$ changes over some edge. This proves the first assertion of the theorem. For the second assertion, we know that Algorithm \ref{alg:general-alg} outputs the same number of canonical pseudofactors as there are equivalence classes under $\thetahrel$, and we may construct a bijection $f_1$ from the canonical pseudofactors to the $\hat\theta$ equivalence classes, $E(G)/\hat\theta$, which takes each $G_i$ to the $E_i \in E(G)/\hat{\theta}$ that was used to construct it, where $\{G_1,\dots,G_n\}$ is the set of graphs output by the algorithm. We also have a bijection $f_3$ from $[m]/\hat\gamma$ to the canonical partition of $\eta$, since the elements of $[m]/\hat\gamma$ were used to form that partition. Thus, the mapping $f = f_3 \circ f_2 \circ f_1$ is a bijection from the canonical pseudofactors of $G$ to the canonical partition of $\eta$.
\end{proof}


\begin{thm}
\label{thm:structure}
Let weighted graph $G$ have canonical pseudofactors $G_1, \dots, G_{n}$. Let $\eta$ be an $m$-dimensional Hamming embedding of $G$ with canonical partition $\eta^1, \dots, \eta^{n}$. Assume without loss of generality that the natural bijection of Theorem \ref{thm:bijection} maps $G_i$ to $\eta^i$ for each $i, 1 \le i \leq  n$. Then $\eta^i$ is a Hamming embedding of $G_i$ for each $i, 1 \le i \leq  n$. From this, we conclude that $G$ is Hamming embeddable if and only if each $G_i$ is Hamming embeddable.
\end{thm}

\begin{proof}
%Fix any two vertices $u,v \in V(G)$.
%We know that the canonical embedding is isometric, so 
%\[ d_G(u,v) = \sum_{i=1}^n d_{G_i}(g_i(u), g_i(v)), \]
%Because $\eta$ is an isometric embedding of $kG$, we also have that
%\[ k\cdot d_G(u,v) = d_{\eta}(u, v) = \sum_{i=1}^n d_{\eta^i}(u, v). \]
From Theorem \ref{claim:pseudofactor5}, we can construct an isometric embedding of $G$ into its canonical pseudofactors, $\pi : V(G) \to V(\prod_{i=1}^n G_i)$, where $\pi = (\pi_1, \dots, \pi_{n})$.

Fix any two vertices $u,v \in V(G)$ and consider a shortest path $P$ from $u$ to $v$.
For each pseudofactor $G_i$, let $E_i$ be the equivalence class under $\hat\theta$ from which $G_i$ was generated and let $c_i$ be the sum of the edge weights for edges along $P$ that are in $E_i$. Because the image of $P$ in $G_i$ is a path, each $d_{\pi_i}(u,v) \le c_i$. Further, each edge along $P$ contributes to exactly one $c_i$, so we have 
\[ d_G(u,v) = \sum_{i=1}^{n} c_i = \sum_{i=1}^{n} d_{\pi_i}(u,v), \]
where the second equality is due to the fact that $\pi$ is an isometric embedding. Thus each $d_{\pi_i}(u,v) = c_i$.
Now take $\eta^i$, for which $w(e)$ digits change across any edge $e \in E_i$ and no digits change across any other edge. Then $d_{\eta^i}(u,v) \le c_i$. In fact, we have
\[ d_G(u,v) = \sum_{i=1}^n c_i = \sum_{i=1}^{n} d_{\eta^i}(u, v), \]
where again the second equality is because $\eta$ is an isometric embedding. As before, this implies that $d_{\eta^i}(u, v) = c_i$. 
Thus, $d_{\eta^i}(u, v) = d_{\pi_i}(u,v)$ as desired. Note that $G_i$ has a single Hamming embedding $\tilde\eta^i$ that satisfies $\eta^i = \tilde\eta^i \circ \pi_i$.

Clearly, if $G$ is Hamming embeddable then we may use the above process to construct Hamming embeddings of each pseudofactor. Similarly, if every pseudofactor is Hamming embeddable, we may concatenate Hamming embeddings of each pseudofactor to get a Hamming embedding of $G$. This proves the final statement of Theorem \ref{thm:structure}.
\end{proof}


\begin{cor}
\label{cor:structure-hypercube}
A weighted graph $G$ is hypercube embeddable if and only if each of its canonical pseudofactors is hypercube embeddable.
\end{cor}

\begin{proof}
If $G$ has a hypercube embedding $\eta$, then each element of the canonical partition of $\eta$ is also a hypercube embedding. Thus each canonical pseudofactor of $G$ is hypercube embeddable because it has a hypercube embedding formed from an element of the canonical partition of $\eta$. Conversely, if each canonical pseudofactor of $G$ has a hypercube embedding, these may be concatenated to form a hypercube embedding of $G$.
\end{proof}

\begin{cor}\label{cor:number-embeddings}
Given a weighted graph $G$, the number of non-equivalent Hamming embeddings of $G$ is the product of the number of non-equivalent Hamming embeddings of each of its pseudofactors. Similarly, the number of non-equivalent hypercube embeddings of $G$ is the product of the number of non-equivalent hypercube embeddings of each of its pseudofactors.
\end{cor}

\begin{proof}
Using Theorem \ref{claim:pseudofactor5}, we can construct an isometric embedding of $G$ into its canonical pseudofactors, $\pi : V(G) \to V(\prod_{i=1}^n G_i)$. Let $\pi = (\pi_1, \dots, \pi_{n})$.

Take any two non-equivalent Hamming embeddings $\eta$ and $\zeta$ of $G$. 
Each element $\eta^i$ of the canonical partition of $\eta$ corresponds to a Hamming embedding $\tilde\eta^i$ of $G_i$, with $\eta^i = \tilde\eta^i \circ \pi_i$. 
This is similarly true of $\zeta$. Now if, for all $1 \le i \le n$, $\tilde\eta^i$ is equivalent to $\tilde\zeta^i$, then each $\tilde\eta^i$ can be made identical to $\tilde\zeta^i$ by permuting coordinates and coordinate values. 
Because $\eta^i = \tilde\eta^i \circ \pi_i$ and $\zeta^i = \tilde\zeta^i \circ \pi_i$, this implies that $\eta$ can be made identical to $\zeta$ by the same process, so $\eta$ and $\zeta$ are equivalent. 
Thus, non-equivalent $\eta$ and $\zeta$ must have some $\tilde\eta^i$ not equivalent to $\tilde\zeta^i$. 
That is, any non-equivalent $\eta$ and $\zeta$ will correspond to Hamming embeddings of the $G_i$ that are distinct under equivalence, so the product of the number of non-equivalent Hamming embeddings of the $G_i$ is at least the number of non-equivalent Hamming embeddings of $G$.

Now let $\tilde\eta^1, \dots, \tilde\eta^{n}$ and $\tilde\zeta^1, \dots, \tilde\zeta^{n}$ be such that each $\tilde\eta^i$ and $\tilde\zeta^i$ are Hamming embeddings of $G_i$. Let $\eta^i = \tilde\eta^i \circ \pi_i$ and $\zeta^i = \tilde\zeta^i \circ \pi_i$, and consider the concatenations of the $\eta^i$ and the $\zeta^i$, $\eta = \eta^1\cdots\eta^{n}$ and $\zeta = \zeta^1\cdots\zeta^{n}$. Note that $\eta$ and $\zeta$ form Hamming embeddings of $G$. If $\eta$ and $\zeta$ are equivalent, then $\eta$ may be made identical to $\zeta$ by permuting coordinates and coordinate values. Note that any such permutation must map each coordinate in $\eta^i$ to a coordinate in $\zeta^i$, because the corresponding digits necessarily change across the same edges. This allows the permutation from $\eta$ to $\zeta$ to be decomposed into permutations from $\eta^i$ to $\zeta^i$, so each $\tilde\eta^i$ and $\tilde\zeta^i$ must be equivalent. 
From this, we conclude that, for any $1 \le i \leq  n$, if $\tilde\eta^i$ and $\tilde\zeta^i$ are not equivalent then their corresponding $\eta$ and $\zeta$ generated by the above process are also not equivalent. This indicates that the number of non-equivalent Hamming embeddings of $G$ is not less than the product of the number of non-equivalent Hamming embeddings of the $G_i$. This completes the proof.

This can be proven identically for counting hypercube embeddings, noting that if $\eta$ and $\zeta$ are hypercube embeddings then each element of their canonical partitions is also a hypercube embedding.
\end{proof}


==> hypercube-background.tex <==
Finally, we will also discuss hypercube and Hamming embeddings. For a given graph $G$, a Hamming embedding is a map $\eta: V(G)\rightarrow \Sigma^t$ for a finite alphabet $\Sigma$ and integer $t$ such that distance in the graph corresponds to Hamming distance between the strings. Formally, let $d_H(\cdot,\cdot)$ be the Hamming distance function, or the function that outputs the number of indices on which two strings differ. Then for any $u,v\in V(G)$, $d_G(u,v)=d_H(\eta(u),\eta(v))$. Additionally, we use subscripts to refer to individual letters in the image of $\eta$, and write $\eta = (\eta_1, \dots, \eta_t)$ or, equivalently, $\eta = \eta_1\cdots\eta_t$. The length $t$ of each string is the \emph{dimension} of Hamming embedding $\eta$. When necessary to refer to the coordinates of $\eta$, we use the notation $[t]$ to refer to the set of the first $t$ positive integers. We also note that a Hamming embedding of dimension $t$ is the same as an isometric embedding into the Cartesian product of $t$ complete graphs.

Finally, a \textit{hypercube embedding} is a Hamming embedding with $|\Sigma|=2$. When discussing hypercube embeddings, we will generally use binary strings, or $\Sigma=\{0,1\}$. 

Two hypercube embeddings, $\eta,\eta'$, of dimension $t$ for a graph $G$ are considered equivalent if there exists a permutation $\sigma$ of the the $t$ indices and $t$ functions $\beta_i$ with $\beta_i(l)=l$ or $\beta_i(l)=1-l$ such that $\eta'(u)=\beta_1(\eta_{\sigma(1)}(u))\beta_2(\eta_{\sigma(2)}(u))...\beta_t(\eta_{\sigma(t)}(u))$ for all $u\in V(G)$. A hypercube embedding is unique if it is equivalent to all other hypercube embeddings for that distance metric.
These definitions and concepts will be expanded upon further in the relevant sections, as we discuss their usefulness and calculations of certain properties.

==> hypercube-previous-work.tex <==
Djokovi\'c showed that deciding whether or not a hypercube embedding exists for an unweighted graph can be done in polynomial time \cite{djokovic1973distance} and Winkler showed that deciding if an unweighted graph has a Hamming embedding can also be done in polynomial time \cite{winkler1984isometric}. In fact, a Hamming embedding exists for a graph $G$ if and only if its canonical pseudofactors are all complete graphs, and it is hypercube embeddable if and only if they are all isomorphic to $K_2$. 


In this paper, we will also consider counting the number of hypercube embeddings for a given graph. If a given metric has exactly one unique hypercube embedding, it is called $\ell_1$-rigid. Deza and Laurent show that if a (uniformly weighted) graph is $\ell_1$-rigid, it must be an isometric subgraph of a scaled half-cube \cite{DezaLaurentL1}. They also provide some measure of counting the number of embeddings for complete graphs at a variety of scales, showing that  $2kK_4$ ($K_4$ with edge weights $2k$ for integer $k$) always has $k+1$ unique hypercube embeddings \cite{DezaLaurentText}. In this text, we will discuss how the number of hypercube embeddings for pseudofactors can determine the number of hypercube embeddings for the original graph, which builds on this conclusions to extend it to the Cartesian product of such graphs.
% The authors additionally list a number of embeddings for larger complete graphs such as $K_5$ and $K_6$ and demonstrate that the number of embeddings for any metric on a finite number of points is polynomial in the sum over the distance between all pairs of points. 

==> paper-overview.tex <==
The remainder of this paper is divided into 6 sections. In section 3, we will show that the algorithm used by Graham and Winkler for pseudofactorization of unweighted graphs can also be used to factor weighted graphs that do not have ``extraneous edges", or edges that do not appear on shortest paths. We also show that each graph has an essentially unique irreducible pseudofactorization. As this algorithm runs in polynomial time, we will be able to use it to make conclusions about properties of graphs later on in the paper.

In section 4, we get our primary result as we show that a weighted graph is hypercube embeddable (and analogously Hamming embeddable) if and only if its pseudofactors are. While it is NP-hard to decide if general weighted graphs are hypercube embeddable, some authors have shown that this can be decided in polynomial time for certain classes of weighted graphs. In particular, if a graph is a line graph or a cycle graph \cite{DezaLaurentL1} or if a graph's distances are all in $\{x,y,x+y\}$ for integers $x,y$, at least one of which is odd \cite{LaurentFewDistances}, it is polynomial time decidable. Shpectorov's results also tell us that for graphs with uniform weights, we can decide this in polynomial time \cite{Shpectorov}. This result extends these results by showing that it also takes only polynomial time to decide if isometric subgraphs of the Cartesian products of such graphs are hypercube embeddable (i.e. it is polynomial time to decide for graphs whose pseudofactors fit into one of these categories). The number of graphs that fit into these categories is very restricted, but if future categories of graphs are found to have polynomial time decidability for this property, this result will apply to extend such a result to the isometric subgraphs of Cartesian product of such graphs with each other and with other graphs in this category.


In section 5, we show that a modified version of Feder's algorithm \cite{feder} for factorization works for general weighted graphs. In section 6, we introduce our method for analyzing runtimes the algorithms presented here and conclude that the given algorithms run in $O(|E|^2)$ time plus the time to find all pairs shortest paths (APSP) distances. Using current APSP bounds, this is $O(|E|^2+|V|^2\log\log|V|)$ time total. Then in section 7, we present a modified version of Feder's algorithm \cite{feder} for pseudofactorization and show that this algorithm can find the irreducible pseudofactorization of a weighted graph in as little as $O(|V||E|)$ time plus the time to find APSP distances, giving  $O(|V||E|+|V|^2\log\log|V|)$ time total under current bounds \cite{apsp}. Finally, in section 8 we will add final thoughts on these topics and list some open questions.



==> pseudofactorization-background.tex <==
% \subsection{Pseudofactorization}

In \cite{graham1985isometric}, Graham and Winkler define this concept. (Notably, they refer to this process as \textit{factorization}, but we have changed the name in order to distinguish from the concept of factorization used by other authors and addressed here.) Definition \ref{def:pseudo-fact-unw} defines pseudofactorization for unweighted graphs in the sense used by Graham and Winkler. In order to use the definition, we further extend our notation for isometric embeddings. Consider an isometric embedding of a graph $G$ into a product of $m$ graphs, $\pi: G\rightarrow \Pi_{i=1}^mG_i$. For each $u\in V(G)$, if $\pi(u)=(u_1,u_2,\ldots,u_m)$, we let $\pi_i(u)=u_i$, or the node in position $i$ of the tuple that $u$ maps to under $\pi$. We additionally let ``$\hookrightarrow$'' mean ``can be isometrically embedded into.''

\begin{definition}\label{def:pseudo-fact-unw}
For a graph $G$, a \textbf{pseudofactorization} of $G$ is a set of graphs $\{G_1,G_2,\ldots,G_m\}$ such that  $G\hookrightarrow \Pi_{i=1}^mG_i$. Additionally, to avoid ``extraneous'' nodes in the product graph, we let $\pi$ be an isometric embedding of $G$ into $\Pi_{i=1}^mG_i$ and require that for each $u_i$ in each $G_i$, there exists some $u\in V$ such that $\pi_i(u)=u_i$.
\end{definition}

We additionally consider an analog to prime graphs for pseudofactorization, which we call \textit{irreducible} graphs, defined in Definition \ref{def:irreducible}.

\begin{definition}\label{def:irreducible}
A graph $G$ is \textbf{irreducible} if all pseudofactorizations of $G$ consist of $K_1$ and $G$ itself.
\end{definition}

Analogously to a prime factorization, we let an irreducible pseudofactorization be a pseudofactorization in which all pseudofactors are irreducible.
Graham and Winkler showed that for each connected unweighted $G$ there is in fact a single irreducible pseudofactorization and thus we can call such a set of graphs the \textit{canonical pseudofactor graphs} or the \textit{canonical pseudofactorization} and the isometric embedding of $G$ into their Cartesian product the \textit{canonical embedding} of $G$ \cite{graham1985isometric, winkler1987metric}.
% . If $\{G_1,G_2,...,G_m\}$ is an irreducible pseudofactorization of $G$, then for any other set of graphs, $\{H_1,H_2,...,H_n\}$, such that $G\hookrightarrow \Pi_{i=1}^nH_i$, there is a partition of the $G_i$ into sets $\Gamma_1,\Gamma_2,...,\Gamma_l$ such that $H_j\hookrightarrow \Pi_{G_i\in \Gamma_j}G_i$ \cite{graham1985isometric, winkler1987metric}. 

We note that in the case of weighted graphs, the previous definition of pseudofactorization implies the non-existence of irreducible pseudofactorizations for many graphs. (An example would be $K_2$, which is isometrically embeddable in the Cartesian product of $x$ copies of $K_2$ scaled by $1/x$ for any integer $x$.) Because of this, we slightly alter the definition of pseudofactorization in a way that is consistent with the definition for unweighted graphs but admits irreducible pseudofactorizations for weighted graphs as well. This definition is presented in Definition \ref{def:pseudo-fact-weighted}.

\begin{definition}\label{def:pseudo-fact-weighted}
A \textbf{pseudofactorization} of a graph $G=(V,E,w)$ is a set of graphs $\{G_1,G_2,\ldots,G_m\}$ such that $G$ is isomorphic to an isometric subgraph of $\Pi_{i=1}^mG_i$. 
\end{definition}

Any $H$ that is a member of some pseudofactorization of $G$ is a \textit{pseudofactor} of $G$. We note that if the original graph and the pseudofactor graphs are restricted to all have all edge weights 1, this definition is identical to Definition \ref{def:pseudo-fact-unw} and we also note that every factor of $G$ is a pseudofactor but the converse is not necessarily true.  Finally, we extend the definition of a parent edge to a \textit{parent edge under an embedding $\pi$}. If $\pi:V(G)\rightarrow V(\Pi_iG_i)$ is an isomorphism from $G$ to an isometric subgraph of $\Pi_iG_i$, then we refer to $\pi_i(u)\pi_i(v)$ as the parent edge of $uv\in E(G)$ under embedding $\pi$. Clearly, in this case $\pi_i(u)\pi_i(v)$ is also the parent edge of $\pi(u)\pi(v)$.
